The trigger and data acquisition system of the FASER experiment

The FASER experiment is a new small and inexpensive experiment that is placed 480 meters downstream of the ATLAS experiment at the CERN LHC. FASER is designed to capture decays of new long-lived particles, produced outside of the ATLAS detector acceptance. These rare particles can decay in the FASER detector together with about 500-1000 Hz of other particles originating from the ATLAS interaction point. A very high efficiency trigger and data acquisition system is required to ensure that the physics events of interest will be recorded. This paper describes the trigger and data acquisition system of the FASER experiment and presents performance results of the system acquired during initial commissioning.

==> contents/hardware/lhc_signals.tex <==
\Anna{For now this is a pure copy of the TP text - however redundant with clock board contribution by Enrique?}

The LHC clock (40.08~MHz) and orbit signal (11.245~kHz) are part of the Beam Synchronous Timing (BST), transmitted to beam instrumentation equipment around the LHC over optical fibers using the TTC system~\cite{TTC}. For FASER, this signal will be received over a single optical fiber by a BOBR VME card~\cite{BOBR} from the LHC beam instrumentation group, which extracts the LHC clock and orbit signal to two front panel LEMO connectors. It also provides additional information, such as the global time and accelerator mode over the VME bus, but this is not foreseen to be used. 

The LHC clock provided by the BOBR has a non-negligible jitter, changes during the ramp of the LHC, and is not guaranteed to be continuous. The clock will therefore pass through a Si5344 jitter attenuating clock  multiplier chip~\cite{Si5344} mounted on an evaluation board in the VME crate. This provides a ultra low-jitter clock (90~fs), which tracks the LHC clock at a programmable speed, provides a holdover clock in case the input clock disappears, and provides a zero delay mode that ensures the clock is always at the same delay with respect to the beam interactions. Daily and seasonal variations of up to several ns in the phase of the clock is expected, due primarily to ground temperature variations, and the absolute timing offset will therefore need to be monitored and calibrated with high-energy muons from the IP.

The orbit signal provides a 25~ns pulse once per turn of the LHC. It will be sent directly to the input of the TLB and used to reset the bunch counters in all of the readout. 

